On-demand quantum state transfer and entanglement between remote microwave cavity memories

Modular quantum computing architectures require fast and efficient distribution of quantum information through propagating signals. Here we report rapid, on-demand quantum state transfer between two remote superconducting cavity quantum memories through traveling microwave photons. We demonstrate a quantum communication channel by deterministic transfer of quantum bits with 76% fidelity. Heralding on errors induced by experimental imperfection can improve this to 87% with a success probability of 0.87. By partial transfer of a microwave photon, we generate remote entanglement at a rate that exceeds photon loss in either memory by more than a factor of three. We further show the transfer of quantum error correction code words that will allow deterministic mitigation of photon loss. These results pave the way for scaling superconducting quantum devices through modular quantum networks.

==> main_figs.tex <==
\begin{figure}[tbp]
    \input{figures/fig1}
\end{figure}

\begin{figure}[tbp]
    \input{figures/fig2}
\end{figure}

\begin{figure}[tbp]
    \input{figures/fig3}
\end{figure}

\begin{figure}[tbp]
    \input{figures/fig4}
\end{figure}
